A Turbo Coding System for High Speed Communications

Conventional turbo codes (CTCs) usually employ a block-oriented interleaving so that each block is separately encoded and decoded. As interleaving and de-interleaving are performed within a block, the message-passing process associated with an iterative decoder is limited to proceed within the corresponding range. This paper presents a new turbo coding scheme that uses a special interleaver structure and a multiple-round early termination test involving both sign check and a CRC code. The new interleaver structure is naturally suited for high speed parallel processing and the resulting coding system offers new design options and tradeoffs that are not available to CTCs. In particular, it becomes possible for the decoder to employ an efficient inter-block collaborative decoding algorithm, passing the information obtained from termination test proved blocks to other unproved blocks. It also becomes important to have a proper decoding schedule. The combined effect is improved performance and reduction in the average decoding delay (whence the required computing power). A memory (storage) management mechanism is included as a critical part of the decoder so as to provide additional design tradeoff between performance and memory size. It is shown that the latter has a modular-like effect in that additional memory units render enhanced performance due not only to less forced early terminations but to possible increases of the interleaving depth. Depending on the decoding schedule, the degree of parallelism and other decoding resources available, the proposed scheme admits a variety of decoder architectures that meet a large range of throughput and performance demands.

==> conclusion.tex <==
\section{Conclusion}
\hspace*{\parindent} We present a powerful IBPTC-based coding
scheme and propose the associated decoder architecture and
algorithms for high speed communications. Using a multiple-round
termination test and a dynamic memory management scheme, our
decoder yields performance achievable by a conventional turbo
coded system with higher $E_b/N_0$ and much larger decoding
latency. The highly reliable TTs require only a short CRC code
(low overhead) and binary sign checks. The memory management
scheme makes efficient use of the storage space while maintaining
low average decoding latency even at low SNR region. The decoder
structure is such that expanding the decoder memory size increases
the dynamic range of the memory manager or the interleaving span.
Both lead to improved performance.

%The structure of interleaver used implies that the message passing
%range of an iterative decoder is an increasing function of the IBP
%range (span), the numbers of DRs and the number of blocks involved
%in decoding. We show that the system performance improves as the
%number of memory units $M$ increases.

The new coding scheme offers a variety of design options that are
not available to CTCs. It also provides increased degrees of
freedom for the same design option. For the same number of ADUs,
much more flexible decoding schedules are available. Its decoding
is amenable for highly dynamic decoding schedules that are both
distributive and cooperative: sharing all modularized decoding
resources-the ADUs, interleavers/deinterleavers, memory-while
passing information amongst component decoders.

System performance can be improved by using a proper decoding
schedule, increasing the block size, the IBP period, the number of
decoding iterations, the memory space, and the number of blocks
involved in decoding. The design allow tradeoffs amongst
performance, latency, computing and hardware complexities, e.g.,
the block size can be traded for other parameters without
performance loss and lower memory requirement and higher degrees
of parallelism (including memory access) are feasible by
shortening the block size and using more flexible decoding
resource management scheme. Multiple data sequences can be decoded
in parallel and throughput is limited only by the degree of
parallelism bestowed in the design.

Finally, we want to remark that, like some application layer FEC
codes such as raptor code or LT code our proposal is a
stream-oriented scheme. Moreover, since any existing block-wise
interleaver can be regarded as an IBPI with $S=1$, the associated
APP decoders are reusable and, in a sense, our proposal is
backward compatible, which makes the evolution from existing
standard TCs easy and natural.


==> memory_control.tex <==
\section{VTT IBPTC Decoder with Finite Memory Space}
\subsection{Decoding schedule and early terminations}
\hspace*{\parindent}In subsection 2.3, we have demonstrated the
importance of the decoding schedule in minimizing the decoding
delay. Parallel decoding is a popular design option to shorten the
latency. Fig. \ref{fig:memory_manager} (a) shows a multiple
expanding-window zigzag scheduling table for decoding an IBPTC
with interleaver span $S=1$ and four ADUs, denoted respectively by
\textbf{a}, \textbf{b}, \textbf{c} and \textbf{d}. Data blocks
processed in the odd rows are in the original (pre-permutation)
order while those processed in the even rows are in the
interleaved (post-permutation) order. Each dashed or dotted zigzag
curve represents the schedule for an ADU. The symbol
\textbf{x}$_{mn}$ denotes the $n$th DR of the $m$th phase in the
ADU \textbf{x}'s schedule, where a DR represents the APP decoding
of a pre- or post-permuted block and the associated interleaving
or de-interleaving and the $m$th phase refers to the $m$th
parallel line associated with a schedule. Obviously, the $m$th
decoding phase of \textbf{x} is followed by the $(m+1)$th decoding
phase to its right.

Take ADU \textbf{c}'s decoding schedule as an example, its first
DR of the first phase \textbf{c}$_{11}$ corresponds to the first
DR of Block 3 while the first phase' second DR \textbf{c}$_{12}$
corresponds to the second DR of Block 2. \textbf{c}$_{12}$ can be
performed as the scheduling table shows that Blocks 1,2,3 have
been decoded once and the corresponding extrinsic information
output has been inter-block interleaved so that the post-permuted
Block 2 is completely filled and is ready for a new DR. \textbf{c}
finishes its first phase after \textbf{c}$_{13}$ is done. It then
proceeds with the first DR of the next phase \textbf{c}$_{21}$,
i.e., the first DR of Block 7. An ADU can not start a new DR until
the DR on its left is completed, e.g., \textbf{a}$_{2k},\ k>2$
cannot start unless the DR corresponding to \textbf{d}$_{12}$ is
finished.

As mentioned at the end of subsection 2.1, an ADU can make both
regular and extended early termination decisions (ETDs) in odd
rows' DRs only unless a non-CRC-based TT is used. For DRs in even
rows, however, extended ETDs are still feasible. For example, in
\textbf{a}$_{23}$ ( \textbf{c}$_{25}$) we check if block 3 passes
the TT and ET on this block becomes effective if affirmative. ADU
\textbf{a} (\textbf{c}) then go on to examine whether
\textbf{a}$_{24}$ (\textbf{c}$_{26}$) is necessary by checking
whether both \textbf{c}$_{13}$ and \textbf{d}$_{13}$
(\textbf{a}$_{25}$ and \textbf{b}$_{25}$) pass the TT as well.
When this condition is satisfied, decoding of block 2 is
terminated. On the other hand, in \textbf{b}$_{24}$ no TT is
performed but after de-interleaving its output we run a TT on the
content of \textbf{b}$_{25}$, which contains de-interleaved
outputs from \textbf{d}$_{14}$ and \textbf{a}$_{24}$. Block 2 is
terminated and \textbf{b}$_{25}$ is no longer needed (because of
our schedule and the IBP structure, \textbf{c}$_{25}$ and
\textbf{d}$_{25}$ can not yet be verified although extrinsic
information from \textbf{b}$_{24}$ will be passed on to them) if
the TT result is positive.
\subsection{Memory management}
\hspace*{\parindent}From the above discussion, it is clear that
decoding more than 10 blocks at the same time requires no small
storage area for ASIC or DSP implementation. One should therefore
try to make the most of the memory space available. The decoder
needs space to store (I) received samples undergoing decoding,
(II) extrinsic information, (III) decoded bits to be forwarded to
a higher layer for further processing, and (IV) received samples
awaiting decoding. The management of the last category, assuming
no buffer overflow, requires only an indicator signal to forward a
new block of received samples to the part of the storage area
designated for category (I) that was just released due to a
termination decision.

Category (III) is needed because of the termination variation
across blocks. Its management is straightforward and, besides, it
requires much less storage space. As mentioned in Section 3.1,
assigning the extrinsic values for TT-approved bits a constant
large value is equivalent to using a (special) binary-valued bit
to indicate which partial paths should survive in the APP decoding
process. Hence the decoded bits serve the dual purposes of
representing the decoder decisions and bookkeeping the survivor
paths. The management of categories (I) and (II), however, needs
more efforts and careful considerations.

As long as the probability of termination-defying blocks exists,
practical latency consideration will force us to set an upper
limit $D_{max}$ on the number of DRs. It can be shown that an
unterminated block will prevent the decoder from discarding ${\bf
Y}^3$ associated with those terminated blocks within a $2S$
neighborhood. When the number of blocks that terminate at or
around the $D_{max}$th DR is large so will be the memory required.
Hardware constraint thus imposes another threshold $M_{max}$, the
maximum affordable (allowable) memory units (MU) where an MU
refers to the space for storing categories (I) and (II) associated
with a block of data in the decoder. As our sole purpose is to
demonstrate the critical role a memory manager plays in the
VTT-APP decoder, we assume, for simplicity, that the same number
of bits is used to represent the extrinsic information of a bit
and the corresponding received sample. An MU is thus assumed to
contain $KL$ bits, where a $K$-bit word is used to store either
the extrinsic information or received baseband sample associated
with a transmitted bit.

Because of the termination time variation nature of our decoder, a
memory manager has to take into account both thresholds, $D_{max}$
and $M_{max}$ so as to optimize the performance. When a block has
failed to pass the TT for $D_{max}$ times, it will automatically
be discarded and the MUs storing the corresponding categories (I)
and (II) information are released accordingly. Chances are more
than one block that reach the threshold $D_{max}$ simultaneously
and it is even more likely that the decoder runs out of MUs before
a block reaches the threshold $D_{max}$. For both cases, one
should then give up decoding one or some of the unterminated
blocks. It is both reasonable and intuitively-appearing to
terminate the most ancient block, i.e., the one which has failed
the TT most often. To distinguish from the regular and extended
ETs described in subsection 2.1, we refer to these memory shortage
induced terminations as forced early terminations.

Fig. \ref{fig:memory_manager} (b) shows a finite-memory IBPTC
decoding procedure for one phase of an ADU. The procedure involves
APP decoding, interleaving, deinterleaving, regular and extended
ETDs, and memory check and release. The last two operations are
collectively called the memory management scheme which is
responsible for verifying if there is enough memory during the
decoding process and make a proper memory-release decision if
there is not enough storage space. As there is no computing
involved at all, the complexity is moderate at most.

Denote by $M_F$, $M_d$ and $M_R$, the numbers of free (unused)
MUs, ADUs, and the required MUs for storing one received block. It
follows that $M_R=x$ for a rate $R=1/x$ turbo code. The decoder is
initialized with $M_F = M_{max}$. An ADU begins a phase by
checking if $M_F < M_R$ (Box 2) where the additional MU is for
storing extrinsic information. If $M_F$ does not meet the
condition, the memory manager determines which block is to be
discarded, makes a forced ETD, and releases the related storage
space (Box 4). Otherwise, the decoder moves the received samples
of the new block from where they were saved (in the buffer area)
to the corresponding category (I) MUs (Box 3).

Deciding which block is to be given up is simple and clear since
our decoding schedule allows only a single most ancient block in
its left-most active column at any time. When a forced ETD is made
the ADU makes hard decisions on the block to be discarded and
releases the related categories (I) and (II) MUs. As the discarded
block is always the most ancient block and our decoding schedule
is such that all blocks to its left must have been terminated for
one reason or another, we are left with the problem of dealing
with the $S$ adjacent blocks to its right if they have not been
terminated. At least two alternatives exist for solving this
problem. The first solution, which leads to better performance at
the cost of higher complexity, is to interleave or de-interleave
the extrinsic values for use in decoding the $S$ blocks to its
right without further updates. The second one is to make
hard-decisions (stop any further decoding) on all $S$ blocks
within its (right) span, releasing their category (I) MUs while
keeping their category (II) MUs for use in decoding other related
blocks.

At beginning of each DR, we ask the decoder whether the scheduled
DR is needed (Box 5). Unless the decoder has been notified to
by-pass the ensuing DR, we still have to ask if the space for
storing the extrinsic information of the coming DR is available.
When such a space is not available ($M_F = 0$) the decoder has to
find room for the next DR by discarding the most ancient
unterminated block and following the memory release procedure
described above (Box 7). The operations in Box 9 include those
described in the last paragraph of subsection 2.1. When the TCC
makes a regular or extended ETD, the memory manager releases the
corresponding category (II) and parts of category (I) memory (Box
10), memory release procedure 1) and notifies the decoder that
further decodings on these blocks are no longer necessary.


==> simulation_result.tex <==
\section{Numerical Examples}
\hspace*{\parindent} The simulation results reported in this
section is based on the following assumptions and parameters. The
component code of the rate=1/3 TC, $G(D)=[1, 1+D^2+D^3/1+D+D^3]$,
and the CRC-8(= ``110011011") code used are the same as those
specified in the 3GPP standard \cite{3GPP}. The APP decoder uses
the Log-MAP algorithm and the IBP algorithm of \cite{IBPTC2} while
the interleaving length and span are left as variables; $M_R=3$
MUs and $N=1000$ per computer run are assumed. Except for the
Genie TT, our simulations do not assume perfect block termination.

%We show the influence of the IBPI span in Fig.
%\ref{fig:BER_FER_L=100} for a system using a block length of
%$L=100$ and employing the tail-biting encoding. An IBPI with $S=4$
%or $5$ gives $0.8$ dB and $1.0$ dB performance gain with respect
%to the $S=1$ IBPI at BER=$10^{-6}$ and FER=$10^{-4}$. The two
%cases $S=4$ and $S=5$ give similar performance because their
%corresponding local decoding delays, $(S+1)L=500$ and 600 bits are
%close. This figure tells us that IBPTC is a good candidate coding
%scheme even for short block length applications and its
%performance can be improved by simply increasing the span. The
%fact that increasing $S$ from 2 to 3 does not bring about any
%performance improvement is because 3 is a factor of the component
%code's period \cite{IBPTC,IBPTC2}.

The effects of various TTs on the IBPTC VTT-APP decoder
performance for the system with $S=1$, $L= 400$, $D_{max}=30$ and
(zero-)tail-padding encoding are shown in Figs. \ref{fig:BER}
$\sim$ \ref{fig:AVE_IT}. Multiple-round CRCTT, SCTT and HTT are
considered. For comparison, we include performance curves of the
decoder using the genie TT, that with fixed $20$ and $30$ DRs
($10$ and $15$ iterations) and that of the CTC with block length
$L=800$ using the genie TT with $D_{max}=30$.

BER performance improves as the number of test rounds $m$
increases no matter which TT is used. Fig. \ref{fig:BER} shows
that T1.3 outperforms T1.2 for $E_b/N_0$ greater than 0.3 dB.
Tests using sign-check alone, T2.3 and T2.5, are inferior to other
termination criteria since, as mentioned before, the class of
sign-check tests check if decoded bits converge but can not
guarantee the quality of the tentative decoded vectors. Incorrect
termination decisions will spread false information to the
neighboring blocks through interleaving and result in degraded
performance. T1.3, T3.2, T3.3 and the one with fixed 30 DRs yield
the best performance and they are almost as good as the genie TT.
Using T3.2 for early termination, the IBPTC has $0.4 \sim 0.6$ dB
gain against the CTC for BER=$10^{-5} \sim 10^{-6}$ although the
average decoding delay per DR for both codes are about the same.

%\textcolor[rgb]{1.00,0.00,0.00}{It is interesting to notice from
%Fig. \ref{fig:BER} that the genie TT does not provide the best BER
%performance in the low SNR region. Our explanation about this
%not-so-perfect performance for a perfect termination detector is
%as followings. Although other TTs may give wrong error-free
%indication when there is still few erroneous decoded bits within a
%block, they output the majority of correctly decoded bits as well.
%As the VTT-APP decoder assigns a positive or negative ``infinity"
%soft values to these bits, the IBP structure then pass these
%correct decision values to the neighboring blocks, dominating the
%ensuing decoding decisions on the bits within its interleaving
%span. However the genie TT outputs a dominant soft value only if
%all bits in the tentative decoded vector are error-free,
%postponing the time for correct decisions on the bits in the
%neighboring block.}

Fig. \ref{fig:AVE_IT} shows the average DR performance of various
TTs. Except for the two sign-check tests, all TTs require less
than $20$ or $10$ APP DRs ($10$ or $5$ iterations) when $E_b/N_0$
is greater than $0.2$ or $0.6$ dB . Considering both BER and
average latency performance, we conclude that, among the TTs we
have examined, T3.2 is the best choice for ETDs.

The numerical results presented so far assume no memory
constraint. Fig. \ref{fig:BER_JM} and \ref{fig:AVE_DR_JM} reveals
the impact of finite memory size for the system that employs a
T3.2-aided VTT-APP decoder and the memory management algorithm of
the previous section with block length $L=400$, interleaving span
$S=1$ and $M_d=1$. Fig. \ref{fig:BER_JM} shows BER performance for
different memory constraints. For convenience of comparison, we
also present three cases without memory constraint, one with
$D_{max}=200$, the other two with fixed DRs. It is reasonable to
find that larger memory sizes give better performance. At higher
$E_b/N_0 (> 0.8$ dB), all performance curves converge to the same
one since all VTT-APP decoders finish decoding after only a few
DRs (see also Fig. \ref{fig:AVE_DR_JM}) and memory size is no
longer a problem. The fact that the cases $D_{max}= 100$ with
$100$ MUs, and $D_{max}=30$ with $100$ MUs give almost identical
performance indicates that increasing $D_{max}$ beyond a certain
number (30 in this case) can not improve BER performance and the
memory size becomes the dominant factor. Performance for the
decoder with $D_{max}=200$ and no memory constraint (it can be
shown that $804$ MUs is sufficient for this case, which is at
least eight time larger than that required by other decoders) is
clearly better than the other decoders when $E_b/N_0 < 0.6$ dB but
this edge is gradually diminished after 0.6 dB.

The average DR performance is given in Fig. \ref{fig:AVE_DR_JM}.
For $E_b/N_0 \geq 0.5$ dB, all VTT-APP decoders need less than or
equal to $10$ DRs ($5$ iterations). But when $E_b/N_0 < 0.3$ dB,
the performance curves are distinctly different--if we do not
impose a memory constraint, the average DR will increases
exponentially as $E_b/N_0$ decreases. Most of the computation
effort will be wasted, so is the memory. In other words, at the
low $E_b/N_0$ region, TTs can not offer early terminations.
Imposing a memory constraint and invoking a proper memory
management algorithm do provide a solution that forces early
terminations, saving computing power and memory at the cost of a
small performance loss. Finally, we find that, compared with our
proposed schemes, the two decoders with fixed DRs ($20$ and $30$)
usually need much more memory and DRs.

The effectiveness of various TTs on the performance of a CTC with
$L=800$ are shown in Fig. \ref{fig:TC_BER} and Fig.
\ref{fig:TC_AVD_JM}. $D_{max}=30$ DRs and tail-padding encoding
are assumed. The BER performance of T1.1 improves as the length of
the CRC code increases. T1.1 requires the minimum average DRs at
the cost of BER performance degradation. The performance of T1.2
with CRC-8 is similar to that of T1.1 with CRC-16. T1.3 with CRC-8
already yields performance that is almost identical to that of the
genie TT, so are T2.3 and T3.2. A higher-order TT leads to better
decisions although the BER performance gain diminishes as $m > 2$
for all TTs considered. We also find that the average DRs for T3.2
is only one more than that required by the genie TT while their
BER performance is about the same. When compared with its
performance in IBPTC systems, T3.2 needs one more average DR but
suffers from significant performance loss. However, if we take
into account the BER and latency performance in both CTC and IBPTC
systems, T3.2 is still the best candidate test. It provides better
error detection capability than T1.1 with CRC-24, which confirms
our conviction that a multiple-round test with a short CRC code is
better than a single-round test with a much longer CRC code.


==> system_model.tex <==
\section{System Model and IBP Behavior}
\subsection{System model}
\hspace*{\parindent} Shown in Fig. \ref{fig:system} (a) is a
generic block diagram for a communication system using an IBPTC.
The input data sequence ${\bf X}$ is partitioned into blocks of
the same length, $\{{\bf X}_1,{\bf X}_2,\cdots \}$, where ${\bf
X}_i$ is a row vector of length $L-K_{CRC}$ representing the $i$th
block. They are CRC-encoded into ${\bf W}=\{{\bf W}_1,{\bf
W}_2,\cdots\}$, where ${\bf W}_i=\{w_{i0},w_{i1},\cdots,
w_{i(L-1)}\}$ is a row vector with length $L$. {\bf W} is formed
by padding at the end of each data block parity bits that are the
coefficients of the remainder polynomial $r(x)$ obtained by
dividing a data polynomial associated with a data block by a
binary generator polynomial $g(x)$ of order $K_{CRC}$. Of course,
the degree of $r(x)$ is less than $K_{CRC}$. The corresponding
probability of undetectable error is roughly equal to
$2^{-K_{CRC}}$. In other words, longer CRC codes possess better
error detection capability.


The CRC encoder output ${\bf W}$ and its IBPI-permuted version
${\bf W}'=\{{\bf W'}_1,{\bf W'}_2,\cdots,\}$ are then encoded to
form the coded sequence ${\bf Z}=\{{\bf Z}^1,{\bf Z}^2,{\bf
Z}^3\}$, where ${\bf Z}^i=\{{\bf Z}^i_1,{\bf Z}^i_2,\cdots \}$ and
the superscript $i$ is used to denote the systematic part ($i=1$),
the first encoder's output (parity) sequence ($i=2$) and the
second encoder's output sequence ($i=3$). Fig. \ref{fig:system}
(b) shows the structure of a TC encoder where the only difference
between a CTC and an IBPTC encoders is the interleaver used.


The receiver uses one or multiple APP decoding unit (ADU) like
that shown in Fig. \ref{fig:system} (c) to decode the
corresponding received baseband sequence ${\bf Y}=\{{\bf
Y}^1_1,{\bf Y}^2_1,{\bf Y}^3_1,{\bf Y}^1_2,{\bf Y}^2_2,$ ${\bf
Y}^3_2,\cdots \}$, where ${\bf Y}^i_j$ is the subsequence
corresponding to ${\bf Z}^i_j$; other notations are defined in the
next section. An ADU consists of an APP decoder and a termination
condition checker (TCC). It also performs the corresponding
interleaving or de-interleaving and other related operations but
for simplicity we do not show these operations in the figure.

The TCC applies CRC check and/or other forms of termination tests
(TTs) to verify if the APP decoder output satisfies the
termination criterion. An affirmative answer leads to the decision
to stop decoding (terminate) the block in question and this is the
only possible early termination (ET) opportunity for CTCs. Besides
such regular ETs, however, there are two other ET opportunities
for IBPTCs since no matter whether the decoder output passes the
TT, the corresponding soft output is interleaved or de-interleaved
to the neighboring blocks within the IBP span. The TCC will then
examine each block within the span and check if the content has
been filled with terminated decisions. If such a block is found
the TCC will issue a termination decision accordingly. The TCC can
also run TTs on these neighboring blocks and make a termination
decision. We refer to the latter two ET possibilities as extended
ETs. Note that a decoding iteration consists of two DRs that are
respectively responsible for decoding the pre-permuted
(non-interleaved) ${\bf Z}_j^2$ and post-permuted (interleaved)
blocks ${\bf Z}_j^3$ and CRC check is feasible for pre-permuted
blocks only. Hence in the first DR one can perform both regular
and extended ETs, but in the second DR, only extended ET is viable
unless the TT does not involve a CRC check. Examples are given in
Section 5 to further elaborate this property of IBPTCs.

%For an $n$-block data sequence, an IBPTC can be viewed as a CTC
%with an extended interleaving size. Although such a CTC usually
%requires large encoding and decoding latency, the corresponding
%IBPTC codec latency is only bounded by its ``local" decoding
%delay, which is equal to $(S+1)$ times the fixed block size $L$,
%no matter how long the data sequence is. This is because, as
%mentioned in Section 1, a symmetric IBPI permutes the contents of
%a given block to its immediate neighboring $2S$ blocks only; see
%Fig. 2. More discussion on the latency issue is given in
%subsection 2.3.


\subsection{Graphical representation of an IBPTC}
\hspace*{\parindent}Fig. \ref{fig:factor_graph} is a graphical
representation for the system of Fig. \ref{fig:system} with a
symmetric IBPI of interleaving span $S=1$ and an input data
sequence ${\bf X}$ of five-block duration. The black-, red-,
green- and blue-colored squares represent respectively the
functions of convolution codec, CRC codec, IBPI and the channel
effect. This extended graph is used to describe the iterated
decoding behavior. As one can see, the content of a given block,
say ${\bf W}_2$, is interleaved to parts of itself ${\bf
W}_2^{\prime}$ and the two neighboring blocks ${\bf W}_1^{\prime}$
and ${\bf W}_3^{\prime}$ to its immediate left and right.

At the first DR, the decoder uses ${\bf Y}_i^1$, ${\bf Y}_i^2$ to
decode block ${\bf W}_i$. The extrinsic information of, say ${\bf
W}_1$ and ${\bf W}_5$, is interleaved for use in decoding ${\bf
W}_1^{\prime}$, ${\bf W}_2^{\prime}$ and ${\bf W}_4^{\prime}$,
${\bf W}_5^{\prime}$ in the second DR. It is easy to see that, in
decoding the third block ${\bf W}_3$ at the beginning of the
second iteration, the decoder can use as a priori information some
message passed from all five neighboring blocks. In general, an
IBPTC decoder can exploit information collected from $4SI+1$
adjacent blocks in $I$ iterations while, as will be shown in the
ensuing subsection, the average decoding delay between two output
blocks is kept fixed. This massage passing range expansion
capability implies that an IBP interleaver can have an unbounded
equivalent interleaving depth (size) that is constrained only by
the numbers of turbo decoding iterations and the data blocks
involved in decoding while keeping the interleaving delay per
iteration bounded by its local interleaving depth.

\subsection{The latency issue}

\hspace*{\parindent}Although the interleaving process of an IBPI
is defined by the composition of the intra- and inter-block
permutations, it can be implemented by a single step. The encoder
knows to which position each bit (or sample) in a given block
should be moved and can do so immediately after it receives each
incoming bit. But to encode a given, say the $i$th, interleaved
block ${\bf U}_i'$ into ${\bf X}_i^2$, it has to wait until the
complete $(i+S)$th block is received. The time elapsed between the
instant the encoder receives the first bit of the $i$th block and
the moment when it receives the last bit of the $(i+S)$th block
and outputs its first encoded bit of ${\bf X}_i^2$ is simply
$(1+S)L$-bit durations. By contrast, a CTC with a block size of
$L$ bits has an encoding delay of approximately $L$ bits.

The single-round interleaving (or de-interleaving) delay (SRID) is
proportional to the encoding delay. But the decoding delay is a
much more complicated issue. For the first decoding of each
incoming block, there can be zero waiting time, but for later DRs
the corresponding delays depend on, among other things, the
decoding schedule used. With the same block size, the decoding
delay of the first received block for the CTC is definitely
shorter than that for the IBPTC. But if one considers a period
that consists of multiple blocks (otherwise one will not have
enough blocks to perform inter-block permutation) and takes the
decoding schedule into account, then the average decoding latency
difference can be completely eliminated. This is because the APP
decoder (including the interleaver and deinterleaver) will not
stay idle until all blocks within the span of a given block are
received. Instead, the APP decoder will perform
decoding-interleaving or deinterleaving operations for other
blocks according to a predetermined decoding schedule before it
can do so for the given block (and the given DR).

If we define the total decoding delay (TDD) as the time span
between the instant a decoder receives the first input sample
(from the input buffer) and the moment when it outputs its last
decision then both the IBP and classic approaches yield the same
TDD even if only one APP decoder is used. We use the following
example and Fig. \ref{fig:scheduling_comparison} to support our
claim; its generalization is straightforward.

Suppose we receive a total of 7 blocks of samples (in a packet,
say) and want to finish decoding in 2 iterations (4 DRs). One can
easily see from Fig. \ref{fig:scheduling_comparison} that a
classic TC decoder would output the first decoded block in 4 $DT$
cycles, where $DT$ is the number of cycles needed to perform a
single-block APP decoding plus SRID. The IBPTC decoder, on the
other hand, needs 10 DT cycles to output its first decoded block.
However, if one further examines the decoding delays associated
with the remaining blocks, then one finds they are 8, 12, 16, 20,
24, and 28 DT cycles for the CTC decoder while those for the IBPTC
decoder are 14, 18, 22, 25, 27 and 28 DT cycles, respectively. So
in the end, both approaches reach the final decision at the same
time.

It can be shown that, for a decoder with $2N$ DRs and $S=1$, both
decoders result in a constant delay of $2N$ DT cycles between two
adjacent output blocks, except for the first block and the last
$2N-1$ blocks. For an $S=1$ IBPTC, the decoder requires a
first-block decoding delay (FBDD) of $N(1+2N)$ DT cycles while the
FBDD for the classic TC is only $2N$ DT cycles. The inter-block
decoding delays (IBDD, i.e., decoding latency between two
consecutive output blocks) for the last $2N-1$ output blocks of an
IBPTC decoder using a decoding schedule similar to that shown in
Fig. 3 (e.g., the one shown in Fig. \ref{fig:memory_manager} (a))
form a monotonic decreasing arithmetic sequence $\{2N-1, 2N-2,
\cdots, 1\}$ (in DT cycles). The IBDD of a CTC decoder remains a
constant $2N$ DT cycles. On the average, both codes give the same
IBDD.


The above assessment on the encoding/decoding delay is made under
the assumptions that both codes use the same block size $L$, no
early termination mechanism is applied, and a single APP decoder
is used. As was mentioned in the previous subsection, an IBPTC has
an equivalent interleaving depth that grows as the number of
iterations increases, hence \cite{Zheng04} with an identical block
size an IBPTC always outperforms its classic counterpart. In other
words, an IBPTC requires a smaller block size and thus less
decoding delay to achieve the same performance. The IBPTC is also
naturally suited for parallel decoding. An example of decoding an
IBPTC with multiple APP decoders is given in Section 5; see Fig.
\ref{fig:memory_manager} (a). Although both IBPTCs and CTCs can
use multiple decoders for parallel decoding and apply an early
termination method to shorten the decoding latency, we will
explain in the next section and prove numerically in Section 6
that the former class does derive much more benefits.


Before proceeding to the main discourse, it is worthwhile to
recapture an alternative viewpoint on the concepts of IBP based on
the the above example. For a CTC with block size of $7L$ bits, the
FBDD is 28 DT cycles. But if one divides a $7L$-block into 7
subblocks and a special interleaver which performs successive
intra-subblock and inter-block permutations on these subblocks,
the corresponding decoding delays in DT cycles for these subblocks
are 14, 18, 22, 25, 27, and 28, respectively. Therefore, although
both code structures result in identical TDD the IBPTC structure
is able to supply partial decoded outputs much earlier. This
feature, when combined with suitable decoding schedule and
implementation resources, become very beneficial for high
throughput applications.

